Domain Invariant Adversarial Learning

The phenomenon of adversarial examples illustrates one of the most basic vulnerabilities of deep neural networks. Among the variety of techniques introduced to surmount this inherent weakness, adversarial training has emerged as the most effective strategy for learning robust models. Typically, this is achieved by balancing robust and natural objectives. In this work, we aim to further optimize the trade-off between robust and standard accuracy by enforcing a domain-invariant feature representation. We present a new adversarial training method, Domain Invariant Adversarial Learning (DIAL), which learns a feature representation that is both robust and domain invariant. DIAL uses a variant of Domain Adversarial Neural Network (DANN) on the natural domain and its corresponding adversarial domain. In the case where the source domain consists of natural examples and the target domain is the adversarially perturbed examples, our method learns a feature representation constrained not to discriminate between the natural and adversarial examples, and can therefore achieve a more robust representation. DIAL is a generic and modular technique that can be easily incorporated into any adversarial training method. Our experiments indicate that incorporating DIAL in the adversarial training process improves both robustness and standard accuracy.

==> figures/conclusion.tex <==
In this paper, we investigated the hypothesis that domain invariant representation can be beneficial for robust learning. With this idea in mind, we proposed a new adversarial learning method, called \textit{Domain Invariant Adversarial Learning} (DIAL) that incorporates Domain Adversarial Neural Network into the adversarial training process.
% where the natural examples act as our source domain, and the corresponding adversarial examples act as our target domain. 
The proposed method is generic and can be combined with any network architecture in a wide range of tasks. Our evaluation process included strong adversaries 
%(e.g., AA)
, unforeseen adversaries 
%(e.g., $\ell_{1}$, $\ell_{2}$)
, unforeseen corruptions, transfer learning tasks, and ablation studies. Using the extensive empirical analysis, we demonstrate the significant and consistent improvement obtained by DIAL in both robustness and natural accuracy compared to other defence methods on benchmark datasets.
%under various attack settings.


==> includes.tex <==

% %%%%%%%% ICML 2022 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%

% \documentclass[nohyperref]{article}

% % Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% % hyperref makes hyperlinks in the resulting PDF.
% % If your build breaks (sometimes temporarily if a hyperlink spans a page)
% % please comment out the following usepackage line and replace
% % \usepackage{icml2022} with \usepackage[nohyperref]{icml2022} above.
\usepackage{hyperref}


% % Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

\RequirePackage{algorithm}
\RequirePackage{algorithmic}

% % For theorems and such
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{mathtools}
% \usepackage{amsthm}

% % if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % THEOREMS
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}

% % Todonotes is useful during development; simply uncomment the next line
% %    and comment out the line below the next line to turn off comments
% %\usepackage[disable,textsize=tiny]{todonotes}
% \usepackage[textsize=tiny]{todonotes}

% %%%%%%%%%%% end ICML %%%%%%%%%%%%%%%%%%


\usepackage{multirow}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{xcolor}         % colors

%%%%%%%%%%%%%% Custom %%%%%%%%%%%%%%%%%%%%
% \usepackage{subcaption}
\usepackage{graphicx}
% \bibliographystyle{plain}
\usepackage{amsmath}
\usepackage{float}

% \newcommand{\E}{\mathbb{E}}
% \renewcommand{\P}{\mathbb{P}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calH}{\mathcal{H}}

% \newcommand{\sign}{\operatorname{sign}}

\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\sqprn}[1]{\left[ #1 \right]}
\newcommand{\norm}[1]{\Vert #1 \Vert}


\newcommand{\calL}{\mathcal{L}}

% \usepackage{algpseudocode}
% \usepackage[linesnumbered, ruled, vlined]{algorithm2e}
\usepackage{setspace}


\newcommand{\DIAL}{\operatorname{DIAL}}
\newcommand{\nat}{\operatorname{nat}}
\newcommand{\rob}{\operatorname{robust}}
\newcommand{\robloss}{\operatorname{rob}}
\newcommand{\adv}{\operatorname{adv}}
\newcommand{\boundary}{\operatorname{boundary}}
\newcommand{\kl}{\operatorname{KL}}
\newcommand{\ce}{\operatorname{CE}}
\newcommand{\bce}{\operatorname{BCE}}
\newcommand{\awp}{\operatorname{AWP}}
\newcommand{\TRADES}{\operatorname{TRADES}}
\newcommand{\disc}{\operatorname{disc}}


\newcommand{\ak}[1]{{\bf[AK: #1]}}
\newcommand{\ml}[1]{{\bf[ML: #1]}}
\newcommand{\hide}[1]{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

